Noise-Adaptive Confidence Sets for Linear Bandits and Application to Bayesian Optimization

Adapting to a priori unknown noise level is a very important but challenging problem in sequential decision-making as efficient exploration typically requires knowledge of the noise level, which is often loosely specified. We report significant progress in addressing this issue for linear bandits in two respects. First, we propose a novel confidence set that is `semi-adaptive' to the unknown sub-Gaussian parameter $\sigma_*^2$ in the sense that the (normalized) confidence width scales with $\sqrt{d\sigma_*^2 + \sigma_0^2}$ where $d$ is the dimension and $\sigma_0^2$ is the specified sub-Gaussian parameter (known) that can be much larger than $\sigma_*^2$. This is a significant improvement over $\sqrt{d\sigma_0^2}$ of the standard confidence set of Abbasi-Yadkori et al. (2011), especially when $d$ is large or $\sigma_*^2=0$. We show that this leads to an improved regret bound in linear bandits. Second, for bounded rewards, we propose a novel variance-adaptive confidence set that has much improved numerical performance upon prior art. We then apply this confidence set to develop, as we claim, the first practical variance-adaptive linear bandit algorithm via an optimistic approach, which is enabled by our novel regret analysis technique. Both of our confidence sets rely critically on `regret equality' from online learning. Our empirical evaluation in diverse Bayesian optimization tasks shows that our proposed algorithms demonstrate better or comparable performance compared to existing methods.

==> defs-kjun-v5-overleaf.tex <==
%--- synctex
\synctex=1
% \pdfoutput=1  % for arxiv submission

%--- prints out an error when the symbol is already defined.
\def\safedef#1{% 
   \ifx#1\undefined
      \expandafter\def\expandafter#1%
   \else
      \errmessage{The \string#1 is defined already}% 
      \expandafter\def\expandafter\tmp
   \fi
}

%--- math better math font
\usepackage{amsthm,amsmath,bbm,amsfonts,amssymb}
\usepackage{dsfont} % require for using \mathds{1}
\usepackage{mathtools}
\usepackage{commath}
\usepackage{eqnarray}
\mathtoolsset{showonlyrefs=false}
\allowdisplaybreaks % This allows breaking multi-line equations

%--- font and spacing
\usepackage{xspace}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage[usenames,dvipsnames]{xcolor} % for color names

%--- links
\usepackage{hyperref,url}
%\usepackage{cleveref} % must be loaded after amsthm

%--- floating objects
\usepackage{wrapfig}
\usepackage[export]{adjustbox}
\safedef\imagetop#1{\vtop{\null\hbox{#1}}} % adjusting location of box in table
\usepackage{graphicx,tabularx}
\usepackage{multirow,hhline}% http://ctan.org/pkg/multirow
\usepackage{booktabs}% to use \midrule for drawing a horizontal line in align environment
\usepackage{pbox} % new line in a table cell -- http://tex.stackexchange.com/questions/2441/how-to-add-a-forced-line-break-inside-a-table-cell
\usepackage{algorithm,algorithmic}

%- for vertical alignment of includegraphics
%- http://tex.stackexchange.com/questions/101858/make-two-figures-aligned-at-top
\usepackage[export]{adjustbox}

%--- etc
%\usepackage{capt-of}
%\newcommand{\fix}{\marginpar{FIX}}
%\newcommand{\new}{\marginpar{NEW}}

\usepackage{enumitem}
%\usepackage{etoolbox}


% define your comment color here
\newcommand{\kwang}[1]{{ \color[rgb]{1,0.279,0.998} #1 }}
\newcommand{\kw}[1]{{ \color[rgb]{1,0.279,0.998} #1 }}
\newcommand{\kj}[1]{{\color{RedOrange}[KJ: #1]}}
\newcommand{\fo}[1]{{\color{Violet}[FO: #1]}}
\newcommand{\my}[1]{{\color{ForestGreen}[FO: #1]}}
\newcommand{\gray}[1]{{ \color[rgb]{.6,.6,.6} #1 }}
\newcommand{\blue}[1]{{\color[rgb]{.3,.5,1}#1}}
\newcommand{\kjblue}[1]{{\color[rgb]{.3,.5,1}#1}}
\newcommand{\tblue}[1]{{\color[rgb]{0,0,1}#1}} % 'the' blue
\newcommand{\grn}[1]{{\color{ForestGreen}#1}}
\newcommand{\org}[1]{{\color{Orange}#1}}
\newcommand{\vio}[1]{{\color{Violet}#1}}
\newcommand{\red}[1]{{\color[rgb]{1,.1,.1}#1}}
\newcommand{\gr}[1]{{\color[rgb]{.8,.8,.8}#1}}

\newcommand{\clb}[1]{{\color{blue}#1}}
\newcommand{\clg}[1]{{\color{green}#1}}
\newcommand{\clr}[1]{{\color{red}#1}}
\newcommand{\clc}[1]{{\color{cyan}#1}}

%---------- setup theorem environment
\usepackage{framed}
\usepackage[most]{tcolorbox}
\definecolor{kjgray}{rgb}{.7,.7,.7}

\newtheoremstyle{kjstyle}
{1ex} % Space above
{\topsep} % Space below
{\itshape} % Body font
{} % Indent amount
{\bfseries} % Theorem head font
{.} % Punctuation after theorem head
{.5em} % Space after theorem head
{} % Theorem head spec (can be left empty, meaning `normal')

\newtheoremstyle{kjstyle2}
{.0em} % Space above
{.0em} % Space below
{\itshape} % Body font
{} % Indent amount
{\bfseries} % Theorem head font
{.} % Punctuation after theorem head
{.5em} % Space after theorem head
{} % Theorem head spec (can be left empty, meaning `normal')


\newtheoremstyle{kjstylenoitalic}
{1ex} % Space above
{\topsep} % Space below
{} % Body font
{} % Indent amount
{\bfseries} % Theorem head font
{.} % Punctuation after theorem head
{.5em} % Space after theorem head
{} % Theorem head spec (can be left empty, meaning `normal')

\tcbset{kjboxstyle/.style={title={},breakable,colback=white,enhanced jigsaw,boxrule=1.3pt,sharp corners,colframe=kjgray,boxsep=0pt,coltitle={black},attach title to upper={},left=.8ex,bottom=.4em}}    

\tcbset{kjboxstylec/.style={title={},breakable,colback=white,enhanced jigsaw,boxrule=1.3pt,sharp corners,colframe=kjgray,boxsep=0pt,coltitle={black},attach title to upper={},before skip=1.5ex,left=.8ex,bottom=.4em,top=0.4em,enlarge top by=-0.3em,enlarge bottom by=-0.3em}}    
%    ,title after break={Lemma \thelemma\ (continued)}}
%}

\newtheorem{theorem}{Theorem}

\theoremstyle{kjstyle}\newtheorem{thm}{Theorem}
\AtBeginEnvironment{thm}{\begin{tcolorbox}[kjboxstyle]}%
  \AtEndEnvironment{thm}{\end{tcolorbox}}%
\theoremstyle{kjstyle}\newtheorem{lem}[thm]{Lemma}
\AtBeginEnvironment{lem}{\begin{tcolorbox}[kjboxstyle]}%
  \AtEndEnvironment{lem}{\end{tcolorbox}}%
%\theoremstyle{kjstyle}\newtheorem{lem}[thm]{Lemma}
%\AtBeginEnvironment{lem}{\begin{tcolorbox}[kjboxstyle]}%
%  \AtEndEnvironment{lem}{\end{tcolorbox}}%
\theoremstyle{kjstyle}\newtheorem{prop}[thm]{Proposition}
\AtBeginEnvironment{prop}{\begin{tcolorbox}[kjboxstyle]}%
  \AtEndEnvironment{prop}{\end{tcolorbox}}%
\theoremstyle{kjstyle}\newtheorem{cor}[thm]{Corollary}
\AtBeginEnvironment{cor}{\begin{tcolorbox}[kjboxstyle]}%
  \AtEndEnvironment{cor}{\end{tcolorbox}}%

\theoremstyle{kjstyle}\newtheorem{defn}{Definition}
\AtBeginEnvironment{defn}{\begin{tcolorbox}[kjboxstyle]}%
  \AtEndEnvironment{defn}{\end{tcolorbox}}%

\theoremstyle{kjstyle}\newtheorem{ass}{Assumption}
\AtBeginEnvironment{ass}{\begin{tcolorbox}[kjboxstyle]}%
  \AtEndEnvironment{ass}{\end{tcolorbox}}%
\renewcommand\theass{A\arabic{ass}}

\theoremstyle{kjstyle}\newtheorem{conj}{Conjecture}
\AtBeginEnvironment{conj}{\begin{tcolorbox}[kjboxstyle]}%
  \AtEndEnvironment{conj}{\end{tcolorbox}}%


\theoremstyle{kjstyle}\newtheorem{question}{Question}
\AtBeginEnvironment{question}{\begin{tcolorbox}[kjboxstyle]}%
  \AtEndEnvironment{question}{\end{tcolorbox}}%
% \renewcommand\theass{A\arabic{ass}}

\theoremstyle{kjstylenoitalic}\newtheorem{remark}{Remark}
\AtBeginEnvironment{remark}{\begin{tcolorbox}[kjboxstyle]}%
  \AtEndEnvironment{remark}{\end{tcolorbox}}%
\theoremstyle{kjstylenoitalic}\newtheorem{openp}{Open Problem}
\AtBeginEnvironment{openp}{\begin{tcolorbox}[kjboxstyle]}%
  \AtEndEnvironment{openp}{\end{tcolorbox}}%

\theoremstyle{kjstylenoitalic}\newtheorem{ex}{Example}
\AtBeginEnvironment{ex}{\begin{tcolorbox}[kjboxstyle]}%
  \AtEndEnvironment{ex}{\end{tcolorbox}}%

\theoremstyle{kjstylenoitalic}\newtheorem{prob}{Problem}


%--------------- other ways to create box
\newcommand{\kjunboxold}[1]{\vspace{.5em}\\\fbox{%
    \begin{minipage}{\linewidth}
      \centering #1
    \end{minipage}%
  }\vspace{.5em}}
\usepackage{mdframed}
\usepackage{lipsum}
\definecolor{kjgray}{rgb}{.7,.7,.7}
\makeatletter
\newcommand{\kjunbox}[1]{\vspace{.4ex}
  \begin{mdframed}[linecolor=kjgray,innertopmargin=1.3ex,innerleftmargin=.4em,innerrightmargin=.4em,linewidth=1.3pt]
    #1
  \end{mdframed}%
}
\makeatletter
\newcommand{\kjunboxcenter}[1]{\vspace{.4ex}
  \begin{mdframed}[linecolor=kjgray,innertopmargin=1.3ex,innerleftmargin=.4em,innerrightmargin=.4em,linewidth=1.3pt,userdefinedwidth=.8\linewidth,align=center]
    %[linecolor=black,innerleftmargin=.4em,innerrightmargin=.4em,userdefinedwidth=.8\linewidth,align=center]
    #1
  \end{mdframed}%
}
\makeatother


%--- to remove the space before paragraph : change 3.25ex to ...
\makeatletter
\renewcommand{\paragraph}{%
  \@startsection{paragraph}{4}%
  {\z@}{0.50ex \@plus 1ex \@minus .2ex}{-1em}%
  {\normalfont\normalsize\bfseries}%
}
\makeatother

%------- this makes a border that covers other part of the equation....
%- https://tex.stackexchange.com/questions/72692/highlight-an-equation-within-an-align-environment-with-color-option
\usepackage[customcolors,shade]{hf-tikz} % after {}, (right, below) and then (left, above) offset... I don't know how it works; done by trial-and-error.
\newcommand{\hll}[2]{\tikzmarkin[set fill color=yellow!30]{#1}(0.02,-.08)(-0.02,0.3)#2\tikzmarkend{#1}}

%--------------------- better paragraph environment
\newcommand{\myparagraph}[1]{\paragraph{[#1]}\mbox{}\\}

%---- useful sometimes
\safedef\horizontalline{\noindent\rule{\textwidth}{1pt} }

%--- better table
\usepackage{tabularx} 
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% symbol definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ddefloop#1{\ifx\ddefloop#1\else\ddef{#1}\expandafter\ddefloop\fi}

%- hollow
\def\ddef#1{\expandafter\def\csname #1#1\endcsname{\ensuremath{\mathbb{#1}}}}
\ddefloop ABCDFGHIJKLMNORSTUWXYZ\ddefloop % except for E P V Q

%- c: mathcal
\def\ddef#1{\expandafter\def\csname c#1\endcsname{\ensuremath{\mathcal{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop

%- b: mathbf/boldsymbol
\def\ddef#1{\expandafter\def\csname b#1\endcsname{\ensuremath{{\mathbf{#1}}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop  
\def\ddef#1{\expandafter\def\csname b#1\endcsname{\ensuremath{{\boldsymbol{#1}}}}}
\ddefloop abcdeghijklmnopqrtsuvwxyz\ddefloop  % except for bf, which often causes an issue

%- h: hat
\def\ddef#1{\expandafter\def\csname h#1\endcsname{\ensuremath{\hat{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrsuvwxyz\ddefloop % except for 't'
\def\ddef#1{\expandafter\def\csname hc#1\endcsname{\ensuremath{\hat{\mathcal{#1}}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
\def\ddef#1{\expandafter\def\csname hb#1\endcsname{\ensuremath{\hat{\mathbf{#1}}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop % 
\def\ddef#1{\expandafter\def\csname hb#1\endcsname{\ensuremath{\hat{\boldsymbol{#1}}}}}
\ddefloop abcdefghijklmnopqrstuvwxyz\ddefloop % 

%- t: til
\def\ddef#1{\expandafter\def\csname t#1\endcsname{\ensuremath{\tilde{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefgijklmnpqtsuvwxyz\ddefloop % except for o and h and r
\def\ddef#1{\expandafter\def\csname tc#1\endcsname{\ensuremath{\tilde{\mathcal{#1}}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
\def\ddef#1{\expandafter\def\csname tb#1\endcsname{\ensuremath{\tilde{\mathbf{#1}}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
\def\ddef#1{\expandafter\def\csname tb#1\endcsname{\ensuremath{\tilde{\boldsymbol{#1}}}}}
\ddefloop abcdefghijklmnopqrstuvwxyz\ddefloop % 

%- bar
\def\ddef#1{\expandafter\def\csname bar#1\endcsname{\ensuremath{\bar{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrtsuvwxyz\ddefloop
\def\ddef#1{\expandafter\def\csname barc#1\endcsname{\ensuremath{\bar{\mathcal{#1}}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
\def\ddef#1{\expandafter\def\csname barb#1\endcsname{\ensuremath{\bar{\mathbf{#1}}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
\def\ddef#1{\expandafter\def\csname barb#1\endcsname{\ensuremath{\bar{\boldsymbol{#1}}}}}
\ddefloop abcdefghijklmnopqrstuvwxyz\ddefloop % 

%- war: wide bar
\def\ddef#1{\expandafter\def\csname war#1\endcsname{\ensuremath{\overline{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrtsuvwxyz\ddefloop
\def\ddef#1{\expandafter\def\csname warc#1\endcsname{\ensuremath{\overline{\mathcal{#1}}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
\def\ddef#1{\expandafter\def\csname warb#1\endcsname{\ensuremath{\overline{\mathbf{#1}}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
\def\ddef#1{\expandafter\def\csname warb#1\endcsname{\ensuremath{\overline{\boldsymbol{#1}}}}}
\ddefloop abcdefghijklmnopqrstuvwxyz\ddefloop % 

%- exceptions
\safedef\tilr{\tilde r}
\safedef\bff{{\boldsymbol f}}
\safedef\hbff{{\hat{\boldsymbol f}}}
\safedef\hatt{\hat{t}}
\safedef\tilo{{\tilde{o}}}
\safedef\tilh{{\tilde{h}}}
\safedef\bell{{{\boldsymbol\ell}}}
\safedef\tell{\ensuremath{\tilde{\ell}}} 
\safedef\btell{\ensuremath{\widetilde{\boldsymbol{\ell}}}} 
\safedef\hell{{{\hat\ell}}}

\safedef\rialpha{\ensuremath{{\mathring{\alpha}}}} 
\safedef\riz{\ensuremath{\mathring{z}}} 
\safedef\ribeta{\ensuremath{\mathring{\beta}}} 

%--- generic shortcuts
\newcommand{\fr}[2]{ { \frac{#1}{#2} }}
\newcommand{\tfr}[2]{ { \tfrac{#1}{#2} }}
\newcommand{\til}[1]{{\ensuremath{\tilde{#1}}}}
\newcommand{\wtil}[1]{{\ensuremath{\widetilde{#1}}}}
\newcommand{\wil}[1]{{\ensuremath{\widetilde{#1}}}}
\newcommand{\wbar}[1]{{\ensuremath{\overline{#1}}}}
\newcommand{\war}[1]{{\ensuremath{\overline{#1}}}}
\newcommand{\what}[1]{{\ensuremath{\widehat{#1}}}}
\newcommand{\wat}[1]{{\ensuremath{\widehat{#1}}}}
\newcommand\msf[1]{{\mathsf{#1}}}
\newcommand{\T}{\top}
\safedef\wed{\wedge}
\safedef\tsty{\textstyle}
\safedef\bec{\because}
\newcommand{\nab}{\nabla}
\safedef\cd{\cdot}
\safedef\cc{{\circ}}
\safedef\la{\langle}
\safedef\ra{\rangle}
\safedef\dsum{\ensuremath{\displaystyle\sum}} 
\safedef\der{\ensuremath{\partial}\xspace}
\safedef\llfl{\left\lfloor} 
\safedef\rrfl{\right\rfloor}  
\safedef\llcl{\left\lceil}  
\safedef\rrcl{\right\rceil}  
\safedef\lfl{\lfloor} 
\safedef\rfl{\rfloor}  
\safedef\lcl{\lceil}  
\safedef\rcl{\rceil}  
\safedef\larrow{\ensuremath{\leftarrow}\xspace} 
\safedef\rarrow{\ensuremath{\rightarrow}\xspace} 
\safedef\sm{{\ensuremath{\setminus}\xspace} }
\safedef\grad{\ensuremath{\mathbf{\nabla}}\xspace}  
\safedef\lt{\left}
\safedef\rt{\right}

%- checkmarks.
\definecolor{mygrn}{rgb}{0,.8,0}
\definecolor{myred}{rgb}{.8,0,0}
\newcommand{\mycm}{\textcolor{myred}{\cmark}}
\newcommand{\myxm}{\textcolor{myred}{\xmark}}

%--- greek
\safedef\sig{\sigma}
\safedef\om{\omega}
\safedef\dt{\delta}
\safedef\gam{\gamma}
\safedef\lam{\lambda}
\safedef\kap{\kappa}
\safedef\eps{\varepsilon}
\def\epsilon{\varepsilon}
\def\th{\theta}
\safedef\Lam{\Lambda}
\safedef\Dt{\Delta}
\safedef\Gam{\Gamma}
\safedef\Sig{\Sigma}
\safedef\Th{\Theta} 
\safedef\Om{\Omega}

\usepackage{pgffor}
\safedef\greeksymbols{alpha,beta,gamma,gam,delta,dt,eps,epsilon,zeta,eta,theta,th,iota,kappa,kap,lambda,lam,mu,nu,xi,pi,rho,sigma,sig,tau,phi,chi,psi,omega,om,Gamma,Gam,Delta,Dt,Theta,Th,Lambda,Lam,Pi,Sigma,Sig,Phi,Psi,Omega,Om}
\safedef\greeksymbolsnoeta{alpha,beta,gamma,gam,delta,dt,eps,epsilon,zeta,theta,th,iota,kappa,kap,lambda,lam,mu,nu,xi,pi,rho,sigma,sig,tau,phi,chi,psi,omega,om,Gamma,Gam,Delta,Dt,Theta,Th,Lambda,Lam,Pi,Sigma,Sig,Phi,Psi,Omega,Om} % except for eta

%- prefix b: boldsymbol
\foreach \x in \greeksymbolsnoeta{\expandafter\xdef\csname b\x\endcsname{\noexpand\ensuremath{\noexpand\boldsymbol{\csname \x\endcsname}}}}
\safedef\bfeta{{\boldsymbol \eta}}

%- prefix h, hb: hat, hat bold
\foreach \x in \greeksymbols{\expandafter\xdef\csname h\x\endcsname{\noexpand\ensuremath{\noexpand\hat{\csname \x\endcsname}}}}
\foreach \x in \greeksymbolsnoeta{\expandafter\xdef\csname hb\x\endcsname{\noexpand\ensuremath{\noexpand\hat{\noexpand\boldsymbol{ \csname \x\endcsname}}}}}
\safedef\hbfeta{{\hat{\boldsymbol \eta}}}

%- prefix bar, barb: bar, bar bold
\foreach \x in \greeksymbols{\expandafter\xdef\csname bar\x\endcsname{\noexpand\ensuremath{\noexpand\bar{\csname \x\endcsname}}}}
\foreach \x in \greeksymbolsnoeta{%
\expandafter\xdef\csname barb\x\endcsname{\noexpand\ensuremath{\noexpand\bar{\noexpand\boldsymbol{ \csname \x\endcsname}}}}
}
\safedef\barbfeta{{\bar{\boldsymbol \eta}}}

%- prefix t, tb: tilde, tilde bold
\foreach \x in \greeksymbols{\expandafter\xdef\csname t\x\endcsname{\noexpand\ensuremath{\noexpand\tilde{\csname \x\endcsname}}}}
\foreach \x in \greeksymbolsnoeta{\expandafter\xdef\csname tb\x\endcsname{\noexpand\ensuremath{\noexpand\tilde{\noexpand\boldsymbol{ \csname \x\endcsname}}}}}
\safedef\tbfeta{{\tilde{\boldsymbol \eta}}}

\safedef\dmu{{\dot\mu}}
\safedef\ddmu{{\ddot\mu}}

% %--- space
% \safedef\RR{{\mathbb{R}}}
% \safedef\NN{{\mathbb{N}}}
% \safedef\ZZ{{\mathbb{Z}}}
% \safedef\SS{{\mathbb{S}}}
% \safedef\HH{{\mathbb{H}}} 

%--- math operators
\DeclareMathOperator{\EE}{\mathbb{E}} % ensures the left space is proper (e.g., 2\EE[X])
\DeclareMathOperator{\VV}{\mathbb{V}}
\DeclareMathOperator{\PP}{\mathbb{P}}
\DeclareMathOperator{\QQ}{\mathbb{Q}}
\DeclareMathOperator{\hEE}{\hat{\mathbb{E}}}
\DeclareMathOperator{\Var}{{\text{Var}}}
\DeclareMathOperator{\barln}{\overline\ln}%
\DeclareMathOperator{\tr}{\text{\normalfont tr}}
\DeclareMathOperator{\conv}{\text{\normalfont conv}}

\safedef\clip#1{\wbar{\del{#1}}}
\DeclareMathOperator{\one}{\mathds{1}\hspace{-.1em}}
\safedef\onec#1{\one\cbr{#1}}

% \newcommand{\binom}[2]{{\begin{pmatrix} %- already exists in some package.. (maybe commath)
%     #1 \\ #2
% \end{pmatrix}}}              
\newcommand{\normz}[1]{{\norm[0]{#1}}}
\DeclarePairedDelimiterX{\inp}[2]{\langle}{\rangle}{#1, #2}

%-- relationship operators
\newcommand\declareop[3]{%
  \newcommand#1{%
    \mskip\muexpr\medmuskip*#2\relax
    {#3}%
    \mskip\muexpr\medmuskip*#2\relax
}}
\declareop\capprox{1}{{\sr{\const}{\approx}}} % I think 1 means the amount of space.
\declareop\logapprox{1}{{\sr{\mathsf{log}}{\approx}}} % I think 1 means the amount of space.

\newcommand{\lapp}{\mathop{}\!\lessapprox} 
\newcommand{\gapp}{\mathop{}\!\gtrapprox}
\newcommand{\lsim}{\mathop{}\!\lesssim}
\newcommand{\gsim}{\mathop{}\!\gtrsim}

%---- distribution names
\safedef\Bin{\mathsf{Bin}}
\safedef\Uniform{{\mathsf{Uniform}}}
\safedef\Bernoulli{{\ensuremath{\mathsf{Bernoulli}}}}

%--- string
\safedef\kt{{\mathsf{kt}}}
\safedef\mle{{\mathsf{mle}}}
\DeclareMathOperator{\Supp}{{\mathsf{Supp}}}
\safedef\Approx{{\mathsf{Approx}} }
\safedef\denom{{\mathsf{denom}}}
\safedef\eff{{\mathsf{eff}}}
\safedef\Seff{{S_{\mathsf{eff}}}}
\safedef\opt{{\mathsf{opt}}}
\safedef\pes{{\mathsf{pes}}}
\safedef\faury{{\mathsf{faury}}}
\safedef\nice{{\textsf{nice} } } 
\safedef\ErrPrb{{\mathsf{ErrPrb}}}
\safedef\Seg{{\mathsf{Seg}}}
\safedef\COM{\mathsf{COM}}
\safedef\const{\mathsf{const}}
\safedef\wo{{\ensuremath{\mathsf{wo}}}}
\safedef\Top{\mathsf{Top}}
\safedef\Bot{\mathsf{Bot}}
\safedef\Sim{\mathsf{Sim}}
\safedef\TV{\mathsf{TV}}
\safedef\tmin{{\min}}
\safedef\tmax{{\max}}
\DeclareMathOperator{\rank}{{\text{rank}}}
\DeclareMathOperator{\txspan}{{\text{span}}}
\safedef\kl{{\mathsf{kl}}}
\safedef\err{\mathsf{err}} 
\safedef\logloss{{\mathsf{logloss}}}
\safedef\Ber{{\mathsf{Ber}}}
\safedef\erf{{\text{erf}}}
\safedef\erfc{\mathsf{erfc}}
\safedef\rcF{\ensuremath{\mathring{\cF}}} 
\safedef\Cf{{\ensuremath{{\normalfont{\text{Cf}}}}}}
\safedef\barCf{{\ensuremath{\wbar{\text{Cf}}}}}
\newcommand{\Fb}{{\ensuremath{\text{Fb}}}}
\DeclareMathOperator{\SReg}{{\mathsf{SReg}}}
\DeclareMathOperator{\MisPrb}{{{\mathsf{MisPrb}}}}
\safedef\SR{{\ensuremath{\text{SR}}}\xspace}
\safedef\lin{{\ensuremath{\mathsf{lin}}}}
\newcommand{\FSB}{{\ensuremath{\text{FSB}}}}
\newcommand{\Cr}{{\ensuremath{\text{Cr}}}}
\newcommand{\SE}{{\ensuremath{\text{SE}}}}
\safedef\IC{{\ensuremath{\normalfont{\text{IC}}}}}
\newcommand{\Fs}{{\ensuremath{\text{Fs}}}}
\newcommand{\barFs}{{\ensuremath{\wbar{\text{Fs}}}}}
\safedef\Reward{\ensuremath{\text{Reward}}}
\safedef\poly{\operatorname{poly}}
\safedef\Misid{\operatorname{Misid}}
\safedef\Corral{\ensuremath{\normalfont{\textsc{Corral}}}\xspace}
\safedef\AUL{{\ensuremath{\normalfont{\text{AUL}}}}} 
\safedef\Rel{{\ensuremath{\normalfont{\text{Rel}}}}} 
\safedef\Mis{{\ensuremath{\normalfont{\text{Mis}}}}} 
\safedef\Rad{\ensuremath{\text{\normalfont{Rad}}}} 
\DeclareMathOperator*{\argmax}{arg~max}
\DeclareMathOperator*{\argmin}{arg~min}
\DeclareMathOperator{\diag}{{\text{diag}}}
\DeclareMathOperator{\supp}{{\text{supp}}}
\DeclareMathOperator{\sign}{{\text{sign}}}
\DeclareMathOperator{\KL}{{\mathsf{KL}}}

\safedef\Reg{{\mathsf{Reg}}}
\safedef\Regret{\ensuremath{\normalfont{\text{Regret}}}}
\safedef\Wealth{\ensuremath{\normalfont{\text{Wealth}}}}
\safedef\Active{\ensuremath{\text{Active}}}
\safedef\decomp{\ensuremath{\mbox{decomp}}\xspace}
\safedef\sym{{\ensuremath{\text{Sym}}\xspace}} 
\safedef\suchthat{\ensuremath{\text{ s.t. }}} 


%--- min/max
\newcommand{\hyphen}{{\text{-\hspace{-.06em}}}}
\newcommand\kmax[1]{\mathop{#1\hyphen\max}}
\newcommand\kmin[1]{\mathop{#1\hyphen\min}}

%--- colored checkmarks.
\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\cm}{\ding{51}}%
\newcommand{\gyes}{{\color[rgb]{0,.8,0}\cmark}}
\newcommand{\xmark}{\ding{55}}%
\newcommand{\xm}{\ding{55}}%
\newcommand{\rno}{{\color[rgb]{.8,0,0}\xmark}}
\newcommand{\no}{\mbox{\clr{\ding{55}}}}
\newcommand{\yes}{\mbox{\clg{\ding{51}}}}

%--- add equations above or below.
\newcommand{\ubrace}[2]{{\underbrace{#1}_{\textstyle #2}}}
%\newcommand{\sr}[2]{ {\stackrel{#1}{#2}} }
\newcommand{\sr}{\stackrel}


%--- parenthesis or symbols with parenthesis
\newcommand{\evt}[1]{\envert{#1}}
\newcommand*{\medcup}{\mathbin{\scalebox{1.5}{\ensuremath{\cup}}}}%
\newcommand*{\medcap}{\mathbin{\scalebox{1.5}{\ensuremath{\cap}}}}%
\safedef\bigmid{\,\middle|\,\xspace}
\newcommand{\bmid}{\;\middle|\;}
%- super large parenthesis
\makeatletter
\newcommand{\vast}{\bBigg@{3}}
\newcommand{\Vast}{\bBigg@{4}}
\makeatother

%--- etc.
\safedef\rhoX{{\rho_{\mathcal{X}}}}
\safedef\lammin{{\lambda_{\min}}}
\safedef\elllog{{\ell^{\mathsf{log}}}}
\safedef\lampp{{\lam_\pp}}

%---- for equationarray
%\arraycolsep=1.4pt
%\def\arraystretch{3}
\def\mytag#1{\hfill\text{(#1)}}


%--------- 23-0415
\safedef\resh{\text{resh}}
\safedef\SVD{\text{SVD}}
\safedef\op{{\text{op}}}
\safedef\sT{{*\T}}

\newcommand{\edit}[2]{{\xspace\textcolor{blue}{\sout{#1}}}{ \textcolor{red}{#2}}}
\safedef\Vol{{\text{Vol}}}
\safedef\pp{\perp}

\let\vec\undefined % place it before MnSymbol to prevent an error
\DeclareMathOperator{\vec}{\text{\normalfont vec}}

\def\code{\red{\texttt{\#code}}\xspace}
\safedef\rell{{\mathring{\ell}}}
\safedef\lamI{{\lam I}}
\def\frC{{\mathfrak{C}}}
\def\barSig{{\wbar{\Sig}}}

\def\portfolio{{\text{portfolio}}}
